Bisimulation and Hennessy-Milner Logic for Generalized Synchronization Trees

In this work, we develop a generalization of Hennessy-Milner Logic (HML) for Generalized Synchronization Trees (GSTs) that we call Generalized Hennessy Milner Logic (GHML). Importantly, this logic suggests a strong relationship between (weak) bisimulation for GSTs and ordinary bisimulation for Synchronization Trees (STs). We demonstrate that this relationship can be used to define the GST analog for image-finiteness of STs. Furthermore, we demonstrate that certain maximal Hennessy-Milner classes of STs have counterparts in maximal Hennessy-Milner classes of GSTs with respect to GST weak bisimulation. We also exhibit some interesting characteristics of these maximal Hennessy-Milner classes of GSTs.

==> eptcsdata.tex <==
\providecommand{\firstpage}{35}
\providecommand{\publicationstatus}{K. Peters and S. Tini (Eds.): Combined Workshop on Expressiveness in\\ Concurrency and Structural Operational Semantics (EXPRESS/SOS 2017).\\
EPTCS 255, 2017, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.255.3}{10.4204/EPTCS.255.3}}
\pdfoutput=1

